Multi-player Multi-armed Bandits for Stable Allocation in Heterogeneous Ad-Hoc Networks

Next generation networks are expected to be ultradense and aim to explore spectrum sharing paradigm that allows users to communicate in licensed, shared as well as unlicensed spectrum. Such ultra-dense networks will incur significant signaling load at base stations leading to a negative effect on spectrum and energy efficiency. To minimize signaling overhead, an adhoc approach is being considered for users communicating in the unlicensed and shared spectrums. For such users, decisions need to be completely decentralized as: 1) No communication between users and signaling from the base station is possible which necessitates independent channel selection at each user. A collision occurs when multiple users transmit simultaneously on the same channel, 2) Channel qualities may be heterogeneous, i.e., they are not same across all users, and moreover, are unknown, and 3) The network could be dynamic where users can enter or leave anytime. We develop a multi-armed bandit based distributed algorithm for static networks and extend it for the dynamic networks. The algorithms aim to achieve stable orthogonal allocation (SOC) in finite time and meet the above three constraints with two novel characteristics: 1) Low complexity narrowband radio compared to wideband radio in existing works, and 2) Epoch-less approach for dynamic networks. We establish a convergence of our algorithms to SOC and validate via extensive simulation experiments.

==> Analysisic.tex <==
We will now analyze the performance of $dSOC\_SN$ algorithm and show that it leads to a stable orthogonal configuration. Our main result is the following theorem.

\begin{thm}
\label{thm:SOC_Static}
Consider a network with $K$ channels and $N$ players with channel rewards characterized by $\{\mu_{n,k}\}$ for all $n \in [N]$ and $k \in [K]$. For any $\delta>0$, set $T_{rh}$ as in (\ref{eq:trh}). Then, There exists $T(\delta)$ such that for all $t \geq T_{rh} (\delta)+ T(\delta)$ the probability of system being in an SOC is atleast $1-2\delta$.  
\end{thm}
We prove the result using the following lemma. Its proof is given in the appendix. 
\begin{lemma}
	\label{lma:RanHop_Static}
	Let $\delta \in (0,1)$. If RH sub-phase is run for  $ T_{rh}(\delta) $ number of time slots, then all the users will orthogonalize with probability at least $1-\delta$.  
	where 
	\begin{equation}
	\label{eq:trh}
	  T_{rh}(\delta):=\left \lceil \frac{\log(\delta/K)}{ \log\left(1-1/4K\right)} \right \rceil
	\end{equation}
\end{lemma}  
The lemma guarantees that the players are orthogonalized with probability atleast $1-\delta$ at the end of the RH sub-phase. We next prove the theorem conditioned upon this event. The proof is an adaptation of the proof of Thm $1$ in \cite{lax} to our specific frame structure. 

{\em Outline of Proof of Thm.  \ref{thm:SOC_Static}:}  Note that the block structure is designed such that even if a player's request to swap on a channel is rejected, she still gets to observe a reward sample from that arm (in CS slot). Thus the master gets to explore the arms as if she is the only players in the network. Also, each players gets to observe many samples of each arm as their ranking of the arm is based on the UCB Index given in (\ref{eqn:UCBInd}). 
\noindent
Then, following the same arguments as in the proof of Lemma $1$ in \cite{lax}, if all channels are  sampled at least 
\begin{equation}
\label{eqn:MinSamp}
s_{\min}:=\frac{8 \log t}{\Delta_{\min}^2} 
\end{equation}

many times by round $t$, where 
\[\Delta_{\min}=\min_{n \in [N]} \Delta_n \mbox{ and } \Delta_n= \min_{i,j \in [N], i\neq j} |\mu_{n,i}- \mu_{n,j}|\]
then all the arms will have correct ranking of the arms (with respect to the true means) with probability at least $1-2t^{-4}$, and swaps results in both players moving to their better channels leading to decrease in system potential.

However, for the specific block structures designed for coordination, each player may not get a informative reward sample in each time slot. 
A master in a MB, will get at least $2 + K-1$ samples, while a non-master will get at least $2K-2-2$ samples. Hence over an OHS block consisting of $2K^2$ slots, each player will get at least $(K-1)(2K-4)+ K+1$ informative samples. Also, the minimum number of samples given in (\ref{eqn:MinSamp}) should be satisfied for all channels. Hence, the condition on smallest $t$ such that (\ref{eqn:MinSamp}) holds across all arms is given by
\[t\geq K\frac{2K^2}{(K-1)(2K-4)+ K+1}s_{\min}\geq \frac{16K}{\Delta_{\min}^2}\log t.\]
Again using \cite{lax}[Lemma 1], we can show that the smallest $t$, denoted $t_{\min}$, is finite and satisfies
\[t_{\min} \leq \frac{M-1-\sqrt{(M-1)^2- 4M}}{2}, \mbox{  where } M:=\frac{16K}{\Delta_{\min}^2}.\] 
Thus, for all $t \geq t_{\min}$. Every swap results in both players swapping their channels getting better channel than their current reserved channels and the network potential decrease with probability at least $1-2t_{\min}^2.$

Further note that the maximum value of the network potential is $N(K-1)$ 




==> Experiments.tex <==
\subsection{Synthetic Experiment} \label{simulation}
For synthetic experiments, we consider three algorithms, SCNJ1, SCNJ2 and SCNJ3, separately. For each algorithm, the comparison with the respective myopic algorithm in terms of regret is shown. Then, the effect of $N$ and $K$ on the regret of the proposed algorithms is analyzed.
Each numerical result shown here is the average of the values obtained over 50 independent experiments and each experiment considers a time horizon of 30000 slots. For illustration, we consider $J=2$, $N=\{3,4,5\}$, $K=\{8,10,12,14\}$. The channel busy probability for each $K$ is given by $p_{\lceil \frac{K}{2}\rceil} = 0.5$ and for $i > {\frac{K}{2}}$ and $i < {\frac{K}{2}}$, the gap between the channel busy probability of the $i^{th}$ and $(i+1)^{th}$ channel should be at least 0.07. For instance, for $K=8$, we set $p_i = \{0.29,0.36,0.43,0.5,0.57,0.64,0.71,0.78\}$. For these $p_i$, the values of $T_J$ and $T_O$ are fixed and equal to 1000 and 50, respectively. The value of the $T_C$ is 5000 for $K=8$ and is incremented by 2000 for each increase in $K$. 

\begin{figure*}[!t]
	\centering
	%	\vspace{-5mm}
	\subfloat[]{\includegraphics[scale=0.26]{Final_plots/Fig_3(a).pdf}%
		\label{d1}}
		\hspace{0.25cm}
	\subfloat[]{\includegraphics[scale=0.26]{Final_plots/Fig_3(b).pdf}%
		\label{d2}}
	\hspace{0.25cm}
		\subfloat[]{\includegraphics[scale=0.26]{Final_plots/Fig_3(c).pdf}%
		\label{d3}}	
\caption {Comparison of average regret of SCNJ1 algorithm with (a) Myopic algorithm for $N=4$ and $K$=8, (b) $N=\{3,4,5\}$ and $K$=8, (c) $N=4$ and $K=\{8,10,12,14\}$ at different instants of the horizon. The value of $J$ is fixed and equal to 2.}
\label{fig3}
\vspace{-0.2cm}
\end{figure*}

%\begin{figure*}[!t]
%	\centering
%	%	\vspace{-5mm}
%	\subfloat[]{\includegraphics[scale=0.26]{Final_plots/Fig_4(a).pdf}%
%		\label{d1}}
%		\hspace{0.25cm}
%	\subfloat[]{\includegraphics[scale=0.26]{Final_plots/Fig_4(b).pdf}%
%		\label{d2}}
%	\hspace{0.25cm}
%	\subfloat[]{\includegraphics[scale=0.26]{Final_plots/Fig_4(c).pdf}%
%		\label{d3}}	
%	\caption {Comparison of average regret of SCNJ2 algorithm with (a) Myopic algorithm for $N=3$ and $K$=8, (b) $N=\{3,4,5\}$ and $K$=8, (c) $N=4$ and $K=\{8,10,12,14\}$ at different instants of the horizon. The value of $J$ is fixed and equal to 2.}
%	\label{fig4}
%	\vspace{-0.2cm}
%\end{figure*}
 
% \begin{figure*}[!t]
% 	\centering
% 	%	\vspace{-5mm}
% 	\subfloat[]{\includegraphics[scale=0.26]{Final_plots/Fig_5(a).pdf}%
% 		\label{d1}}
% 	\hspace{0.25cm}
% 	\subfloat[]{\includegraphics[scale=0.26]{Final_plots/Fig_5(b).pdf}%
% 		\label{d2}}
% 	\hspace{0.2cm}
% 	%	\hspace{0.5 mm}
% \subfloat[]{\includegraphics[scale=0.26]{Final_plots/Fig_5(c).pdf}%
% 		\label{d3}}	
% 	\caption {Comparison of average regret of SCNJ3 algorithm with (a) Myopic algorithm for $N=3$ and $K$=8, (b) $N=\{3,4,5\}$ and $K$=8, (c) $N=4$ and $K=\{8,10,12,14\}$ at different instants of the horizon. The value of $J$ is fixed and equal to 2.}
% 	\label{fig5}
% 	\vspace{-0.2cm}
% \end{figure*}
 

  \begin{figure}[!t]
 	\centering
 		\vspace{-5mm}
 	\subfloat[]{\includegraphics[scale=0.2]{Final_plots/Fig_4(a).pdf}%
 		\label{d1}}
 	\subfloat[]{\includegraphics[scale=0.2]{Final_plots/Fig_5(a).pdf}%
 		\label{d2}}
 %	\hspace{0.2cm}
 	%	\hspace{0.5 mm}
% 	\subfloat[]{\includegraphics[scale=0.26]{Final_plots/Fig_5(c).pdf}%
% 		\label{d3}}	
 	\caption {Comparison of average regret of Myopic algorithm with (a) SCNJ2 algorithm, and (a) SCNJ3 algorithm for $N=3$, $J=2$ and $K$=8.}
 	\label{fig5}
 	\vspace{-0.4cm}
 \end{figure}
 

\subsubsection{SCNJ1}
Consider SCNJ1 algorithm designed for the scenario where the SUs can distinguish the collisions with other SUs from the collisions with jammers. Fig. \ref{fig3} (a) compares the regret of the SCNJ1 algorithm and myopic algorithm. The latter refers to the algorithm in which the SUs select the channel via random hopping till $T_C$ followed by orthogonalization and sequential hopping among top $N$ channels till the end of the horizon. As shown in from Fig. \ref{fig3} (a), the average regret incurred by both algorithms is identical till $T_C$ due to identical channel selection approach. After $T_C$ time slots, the SUs in the proposed SCNJ1 algorithm sequentially hops among top $N^*$ channels leading to fewer number of collisions with jammers and hence, lower average regret, than the myopic algorithm.  

Fig. \ref{fig3} (b) shows the comparison of the average regret of the proposed SCNJ1 algorithm for $N=\{3,4,5\}$. Since the probability of collision in random hopping increases with the value $N$, the average regret increases with $N$. After $T_C+T_O$ slots, the SCNJ1 algorithm does not incur regret leading to the constant average regret. Next, the performance of the proposed SCNJ1 algorithm for $K=\{8,10,12,14\}$ and fixed $N=4$ is depicted in Fig. \ref{fig3} (c). As expected, the average regret increase till $T_C$ and is higher for large $K$ due to the higher value of the $T_C$. As expected, SCNJ1 algorithm incurs zero regret after $T_C+T_O$ slots leading to the constant average regret thereafter. 

%Spikes at $T_C$ can be observed in Fig. \ref{fig3} (c) because of the collisions faced by randomly hopping SUs, while orthogonalising into top $N^*$ channels, during $T_O$.
\subsubsection{SCNJ2}
Next, we consider the SCNJ2 algorithm designed for the scenario where the SUs can not distinguish between the collisions with other SUs and the collisions with jammers. Also, it considers coordinating jammers. The Fig. \ref{fig5} (a) compares the regret of the SCNJ2 algorithm and myopic algorithm.
It can be observed that both algorithms incur the same regret till $T_C$ due to random hopping. After $T_C$, the SUs in myopic algorithm orthogonalizes on the top $N+J$ channels followed by sequential hopping. In the SCNJ2 algorithm, the SUs orthogonalizes in the $K$ channels followed by sequentially hopping till $T_C+T_O+T_J$ time slots. Thus, the myopic algorithm incurs lower regret than the SCNJ2 algorithm during this phase. After $T_C+T_O+T_J$ time slots, the SUs in SCNJ2 algorithm sequentially hops in the top $N^*$ channels and hence, does not incur any regret leading to the constant average regret. Its regret is lower since $N^* \leq N+J$ and it guarantees the same value of $N^*$ at each SUs. This is not true for myopic algorithm leading to non-zero regret even after $T_C+T_O+T_J$ slots. We skip the discussion for variable $N$ and $K$ since the plots show identical behavior to those of SCNJ1 algorithm.

%Fig. \ref{fig4} (b) shows the comparison of the average regret of the proposed SCNJ2 algorithm for $N=\{3,4,5\}$. Since the probability of collision in random hopping increases with the value $N$, the average regret is high for large $N$. After $T_C+T_O$ time slots, the slope of the regret plot decreases since the SCNJ2 algorithm guarantees zero collisions among SUs for the next $T_J$ time slots. Thereafter, a spike in the slope of the regret plot is due to the collisions among the SUs and jammers as the SUs try to orthogonalize in the top $N^*$ channels. As expected, the average regret is constant thereafter. Next, the performance of the SCNJ2 algorithm for $K=\{8,10,12,14\}$ and fixed $N=4$ is depicted in Fig. \ref{fig4} (c) which is identical to Fig. \ref{fig3} (c) for the same reasons discussed above.

% As expected, average regret increase till $T_C$ and is higher for large $K$ due to higher value of the $T_C$. As expected, SCNJ1 algorithm incurs zero regret after $T_C+T_O+T_J$ time slots leading to constant average regret. 





\subsubsection{SCNJ3}
At the end, we consider the SCNJ3 algorithm designed for the scenario where the SUs can not distinguish collisions with other SUs from the collisions with jammers and non-coordinating jammers. As shown in Fig.~\ref{fig5}(b), the regret plots are similar to the plots in Fig.~\ref{fig5}(a) except $T_J$ phase where both algorithms have identical regret. This is because the SUs in the SCNJ3 algorithm sequentially hops in the top $N+J$ channels compared to $K$ channels in the SCNJ2 algorithm leading to lower regret in former. 

For all plots, the upper and lower bounds on the regret are tight and do not overlap with that of the Myopic algorithm. This validates the superiority of the proposed algorithms. Next, experimental results on USRP testbed are discussed.
%The plot for comparison of average regret of the proposed SCNJ3 algorithm with the random strategy is shown in Fig. \ref{fig5} (a). Here, in the random strategy, the SUs select the channel using random hoping till $T_C$ i.e. same as SCNJ3 algorithm and then they orthogonalise on $N + J $ channels during $T_O$. After $T_O$ onwards, the SUs sequentially hop on the $N + J $ channels, incurring regret. As evident from \ref{fig5} (a), the performance of the proposed SCNJ3 algorithm and the random strategy are same during $T_O$ and $T_J$ as the SUs orthogonalise and then sequentially hop on $N + J$ channels in both the cases.
%% The performance of the random strategy is better than the proposed SCNJ3 algorithm during $T_C$ to $T_J$ because, in this duration, the SUs sequentially hop on top $N + J $ channels in random strategy while they hop randomly on the top $N + J $ channels in the proposed SCNJ2 algorithm.
%  In Fig. \ref{fig5} (b) and Fig. \ref{fig5} (c), similar trend has been observed as in \ref{fig4} (b) and Fig. \ref{fig4} (c). The decrease in slope during $T_J$ in \ref{fig5} (b) and Fig. \ref{fig5} (c) is because of lesser collisions occured in this duration in comparison to $T_O$ duration. This is due to the fact that during $T_O$, in the proposed SCNJ3 algorithm, the SUs collide with jammers as well as other SUs while during $T_J$, collision occurs between the SUs and jammers only. Spikes at $T_C$ and $T_J$ can be observed in \ref{fig5} (b) and Fig. \ref{fig5} (c) because of the collisions faced by randomly hopping SUs, while orthogonalising into top $N + J$ and $N^*$ channels, respectively. 













 \par










==> Model1.tex <==
In this section, we consider the case where jammers cannot communicate with each other and attack channels independently. This attack is more practical as the jammers can simply use multiple SU terminals and tune them to behave maliciously. However, the downside is that multiple jammers may attack the same channel in a slot, thus reducing their effectiveness. We consider indistinguishable collisions here, if they are distinguishable we can directly apply SCNJ1.

For the case of uncoordinated jammers where the collisions cannot be distinguished, it turns out that one can directly estimate the total number of users in the network, i.e., $N+J$ from an estimate of collision probability. To see this, note that  collision probability conditioned on the event that channels are idle is given by
 \begin{equation} {\label{eq:PC1}}
  Pr(collision) = \left(1-\left(1-1/K \right) ^ {N+J-1} \right).
  \end{equation}
 One can get an estimate for $N+J$ from an estimate of collision probability from the above relation. Though the SUs still cannot know the values of $N$ and $J$, but knowing $N+J$ they can find non-overlapping channels on the top $N+J$ channels and then estimate $J$ from the collision information. Note that in the previous case where jammers coordinated, the SUs cannot know $N+J$, so we took a pessimistic approach and orthogonalized SUs over $K$ channels. Once the SUs orthogonalize on the $N+J$ they can estimate $J$ and subsequently get an estimate of $N$. We next give SCNJ3 given in Algorithm \ref{Algo4} which is a modification of SCNJ2 algorithm for the case of uncoordinated jamming attack. 
 
 \begin{algorithm}[!b] 
 	\SetAlgoLined
 	\SetAlgoRefName{4} 
 	\SetKwInOut{Input}{Input}
 	\Input{$T_C,T_O, T_J, T,K$ }
 	$(\widehat{N+J},\ \{\hat{p}_i\} )= CR2(T_C, K)$ \;
 	$OR(\pi, \widehat{N+J}, T_O)$ \\
 	$(\hat{J},\hat{N}) = JE(\pi,T_J)$ \\
 	$N^*=OP1(\hat{N},\hat{J}, \{\hat{p}_i\})$ \\
 	$OP(\pi, N^*,T)$ 
 	\caption{SCNJ3} \label{Algo4}
 \end{algorithm}

 \subsection{SU Algorithm: SCNJ3}
SCNJ3 algorithm also has four subroutines as in SCNJ2 and they run sequentially. The CR2, OR and JE subroutines are the same as in the SCNJ2 algorithm. At the end of CR2 subroutine, using values of $C$ and $F$ each SU finds an estimate for $N+J$ as $\widehat{N+J}= round \left( 
1 + \frac {\log \left( 1-\frac{C}{F}  \right)} {\log \left(1-\frac{1}{K} \right)}
\right) $. The SUs then find non-overlapping channels on the top $\widehat{N+J}$ channels using the OR subroutine. In the JE subroutine, any collision SUs observe are necessarily from the jammers. JE subroutine is run for  $T_J$ number of time slots and collisions observed in this period is used to estimate $J$ using relation  $\hat{J} = round \left ( \sum_{i=1}^{K} K\frac{O_i}{T_J}\frac{C_{\pi_i}}{F_{\pi_{i}}}\right)$(see \ref{eq:JamEstimate}). Then an estimate for $N$ is obtained from $\hat{N}=\widehat{N+J}-\hat{J}$. Using estimates of $N,J$ and $\{p_i\}$, SUs compute $N^*$=$N+m$ using the program $OP1(N,J, \{p_i\}):$
\begin{equation} \label{eq:optm2} 
			m = \argmax_w\left\{ \begin{array}{cl}
				\hspace{-.3cm} \sum\limits_{i=1}^{N+w}\frac{1-p_{\pi_i}}{N+w}  \left(1-\frac{1}{N+J-1} \right)^J  if \ w \leq J-1\\
				 \hspace{-.3cm}\sum\limits_{i=1}^{N+J-1}\frac{1-p_{\pi_i}}{N+w}\left(1-\frac{1}{N+J-1} \right)^J \hspace{-.2cm}+ \hspace{-.2cm} \sum\limits_{i=N+J}^{N+w}\frac{1-p_{\pi_i}}{N+w} \\ if \ K-N \geq w>J-1. \end{array} \right . 
\end{equation}
Note that (\ref{eq:optm2}) is different from (\ref{eq:optm}). In the case of coordinated jammers, jammers know how many jammers are present ($J$), whereas it is unknown to them when they are  not coordinating. Hence in the latter case after estimating $N+J$, each jammer attacks $N+J-1$ channels. (\ref{eq:optm2}) gives $m$ for which average  throughput is maximum for a SU with jammers attacking as in this case. Finally, OR subroutine is again used to find orthogonal channel assignment from top $N^*$ channels. SUs then continue to hop sequentially according to the indices in ${\pi}$ till the end.

Each Jammer independently runs the CR2 module to get an estimate of $N$ and $J$ and attacks the top $N+J-1$ channels continuously after that.
%
%\begin{algorithm}[]
%\SetAlgoLined
%\SetKwInOut{Input}{Input}
%\Input{$\ T_C,\ T$ }
%
% $r_t = 0,\ C= 0 $ \;
% $O_i = 0 , B_i = 0 \ \forall i \in 1\dots K $ \;
% 
%	\For{$t=1 \dots T_C$}{
%		
%		
%		select $I_t \sim U(1\dots K)$ and transmit on $I_t$ \; $O_{I_t} \leftarrow O_{I_t} + 1$ \;
%		
%		\uIf{ selected channel $I_t$ busy}{$B_{I_t} \leftarrow B_{I_t} + 1, r_t \leftarrow 0 $}
%		\Else { 
%			$F = F + 1$ \;
%
%			\uIf{collision}{$C \leftarrow C + 1,  r_t \leftarrow 0$} 
%			\Else{$r_t \leftarrow 1$}
%		}	
%		
%	}
% set $\hat{p}_i = \frac{B_i}{O_i}  \ \forall i \in 1\dots K$ \;
%
% 
%  $ \widehat{N+J} = round \left( 
%     1 + \frac {\log \left( 1-\frac{C}{F}  \right)} {\log \left(1-\frac{1}{K} \right)}
%\right) $ \;
% $ [\pi]\leftarrow$ top $\widehat{N+J}$ indices in $[K]$ sorted according to $\{\hat{p}_i\}$ \; 
% 
%\NoCaptionOfAlgo
%\caption{Subroutine:CR3} 
%
%\end{algorithm}
%
%
%\begin {algorithm} []
%\SetAlgoLined
%\SetKwInOut{Input}{Input}
%\Input{$ \pi,T_O$  }
% $l = 0 ,s = 0$ \;
%
%$T_1$ = $t +T_O$ \;
%  \For{$t=t+1 \dots T_1 $}{
%   	\uIf{$l=1$}{\If{$channel \ s \ free\ \textbf{and} \ collision$}{
%   	  		
%			$ r_t \leftarrow 1 $ \;
%      
%   	 		}	}
%   	\Else {
%      		select $I_t \sim U(\pi_1\dots \pi_{N})$ \;
%     		\If{$channel I_t \ free\ \ \textbf{and} \ collision$}{
%   	  		$l  \leftarrow 1, s \leftarrow I_t, r_t \leftarrow 1 $ \;
%      
%   	 		}	
%  		}
%        }
%\NoCaptionOfAlgo
%\caption{Subroutine: $OR$ }
%\end{algorithm}
% 
%\begin {algorithm} []
%\SetAlgoLined
%\SetKwInOut{Input}{Input}
%\Input{$N, \ T_J$  }
%   $T_2 = t + T_J $ \;      
%  \For{$t=t+1 \dots T_2$}
%{
% \If{$channel \ s\ free$}{
%	$F=F +1  $ \;
%    \uIf{$collision$}{$C \leftarrow C + 1$} 
%     \Else {$ r_t \leftarrow 1 $}
%      }
% 
%} 
%%      
%$\hat{J} = round \left( \frac{\log\left( 1-\frac{C}{F} \right)}{\log \left(1-\frac{1}{N} \right) }\right)$ \;
%
% \NoCaptionOfAlgo
% \caption{Subroutine: $JE$}
%\end{algorithm}
\subsection{\textbf{Analysis of SCNJ3}}
The regret of the SCNJ3 algorithm is same as the SCNJ2 algorithm. Please refer to \cite{TechReport} for proof of the Theorem 3.
 
%\begin{lemma} \label{thm:le5}
%For any $\theta,\epsilon>0$, $\gamma \in (0,\frac{1}{2})$, $\delta \in [0,1]$, $\epsilon_1=\frac{\gamma}{\exp(1).K}$  after 
%$T_C = max (T_{NE},T_{CR}) $ rounds of random exploration, where $T_{NE}=max\left(\frac{8}{\theta}\ln \left(\frac{4K}{\delta_1}\right),\frac{1}{\epsilon^2_1 \theta}\ln \left(\frac{8K}{\delta_1}\right)\right)$, $ T_{CR} = max \left(8K \ln \left(\frac{4K}{\delta_1}\right),\frac{4K}{\epsilon^2}\ln \left ( \frac{8 \cdot K^2}{\delta_1} \right) \right)$ all SUs will have $\epsilon$ correct ranking of channels and all SUs, can estimate N+J with probability atleast $1-\delta_1$. 
%\end{lemma}
%
%Lemma \ref{thm:le5} gives the number of slots required such that all SUs have $\epsilon$ correct ranking of channels and estimate $N+J$ with high probability $1-\delta_1$. In this case, unlike SCNJ2 we have estimate of $N+J$ as we can solve for $N+J$ given in Eq. (\ref{eq:Pc2}). 
%
%\begin{lemma} \label{thm:le6}
%For any $\delta_2 \in [0,1]$, with $T_O = \frac{\log \left(\frac{\delta_2}{K}\right)}{\log \left(1-\left(1-\frac{1}{K} \right) ^ {K-1} \right)}$, all the SUs hopping randomly on $N+J$ chananels will be on orthogonal channels after $T_O$ with probability atleast $1-\delta_2$.
%\end{lemma}
%
%
%Lemma \ref{thm:le6} guarantess that every SU will be on orthogonal channel conditioned that all SUs have estimate of $N+J$ ,after $T_O$ with confidence $1-\delta_2$, where $\delta_2$ is 
%user defined parameter.
%
%\begin{lemma} \label{thm:le7}
%If all SUs are orthogonalised and sequentially hopping on $K$ channels, then for any $\delta_3 \in [0,1]$, $\epsilon_2= \frac
%{\gamma}{Kexp(1)}$, with $T_J = max\left(\frac{8}{\theta }  \cdot \ln \left(\frac{2K}{\delta_3}\right),\frac{1}{\epsilon^2_2 \theta}\ln \left(\frac{4K}{\delta_3}\right)\right)$, all SUs can estimate $\hat{J}=J$ with probability atleast $1-\delta_3$
%\end{lemma}
%
%Lemma \ref{thm:le7} guarantess that given all SUs are orthogonalised as given in lemma \ref{thm:le6}, each SU estimate $J$ with confidence $1-\delta_3$ after $T_J$ rounds.

\begin{thm}\label{thm:t3}
For all  $\Delta > \epsilon$ and $0 \leq\delta\leq 1$, with probability at least $1-\delta$, the expected regret of $N$ SUs using the SCNJ3 algorithm in the presence of $J$ Jammers after $T_L=T_C+T_O+T_J$ time slots of learning is upper bounded by $NT_L + N^2exp(1)$, where the values of $T_C, T_O,$ and $T_J$ are given in  \ref{eq:TC2}, \ref{eq:TO2}, and \ref{eq:TJ2}, respectively with $\epsilon_1=\epsilon_2=\frac{\gamma}{\exp(1).K}$.
\end{thm}








==> USRP_exp.tex <==
\subsection{USRP Experiment}


The USRP based testbed has been developed to validate the functionality of the proposed work in real radio environment and compare it with the myopic algorithm. Due to limited page constraints, we restrict the discussion to the SCNJ2 algorithm and corresponding myopic algorithm since they consider the most challenging scenario of coordinating jammers with the SUs not capable of distinguishing between the collisions from other SUs and collisions from jammers.

	\begin{figure}[!b]
			\vspace{-0.5cm}
	\centering
	\includegraphics[scale=0.07]{testbed}
	\caption{Proposed USRP based experimental testbed.}
	\label{usrp1}
	\vspace{-0.5cm}
\end{figure}

\begin{figure*}[!h]
	\centering
	%	\vspace{-5mm}
	\subfloat[]{\includegraphics[scale=0.25]{N4J2K8_U.pdf}%
		\label{d1}}
	\hspace{0.5mm}
	\subfloat[]{\includegraphics[scale=0.25]{N5J2K8_U.pdf}%
		\label{d2}}
		\hspace{0.5 mm}
	\subfloat[]{\includegraphics[scale=0.25]{coll.pdf}%
		\label{d3}}	
	\caption{Experimental results on USRP testbed for $J$=2 and $K$=8: a) Total throughput of SUs for $N$=4, b) Total throughput of SUs for $N$=5, and c) Total number of times in \% the SUs face collision with other SUs and jammers for $N$=4 and $N$=5.}
	\vspace{-0.4cm}
	\label{dthr}
	
\end{figure*}

The testbed consists of primary user traffic generator designed using OFDM based transmitter realized in LabView and USRP-2922 from National Instruments for over-the-air transmission as shown in Fig.~\ref{usrp1}. It transmits the signal in one or multiple channels based on their statistics. The first channel is dedicated for synchronization and hence, it is not used by the PUs/SUs/jammers for the transmission. The synchronization has been achieved by switching the corresponding channel from occupied to vacant states or vice-versa in each time slot. Each slot duration ($\Delta t$) is 0.1 second so that channel status can be followed by human eye. Though, $\Delta t$ can be reduced further, the main limiting factor is the latency in the USRP and MATLAB connection. For experiments, the transmission parameters such as the number of OFDM sub-carriers, number of channels, center frequency, and bandwidth are 1024, 8, 935 MHz and 2 MHz, respectively. At the receiver side, SUs and jammers are implemented using MATLAB and USRP N200 from Ettus Research. At each SU or jammer, the channel selected by the underlining algorithm is passed through non-ideal energy detector to check whether it is vacant or occupied. When the channel is vacant and it is not selected by other SUs and jammers, it is assumed that the SU transmits over the channel and transmission is successful. The size of the horizon, $T$, is limited to 7000 due to large $\Delta t$ and each result is averaged over 15 independent experiments.









Consider $N=\{4,5\}$, $J=2$ and $p_i=\{0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9\}$. The values of $T_C$, $T_O$ and $T_J$ are 3000, 50 and 1000, respectively. The Fig.~\ref{dthr} (a) and (b) show the comparison of total throughput, i.e. total number of successful transmissions, at different instants of horizon for $N$=4 and $N$=5, respectively. As expected, all algorithms have same throughput till $T_C$ slots. From $T_C$ till $T_C+T_O+T_J$ slots, the myopic algorithm may offer higher throughput than the proposed algorithm as discussed above. Thereafter, the proposed algorithms outperform myopic algorithm. Here, SCNJ2$^*$ refers to the proposed algorithm without the optimization function in (1) and hence, the SUs sequentially hops among top $N$ channels after $T_C+T_O+T_J$ time slots. The difference in the throughput of the SCNJ2 and SCNJ2$^*$ algorithms show that identifying the subset size of optimum channels is as important as accurate estimation of $N$, $J$ and $p_i$ to achieve higher throughput. As evident from the slope of the plots after $T_C+T_O+T_J$ slots, the difference in the throughput between the proposed and myopic algorithms increases with time. Similar behavior can also be seen in Fig.~\ref{fig3}(a) and Fig.~\ref{fig5}. 
 
 The Fig.~\ref{dthr} (c) shows the total number of collisions faced by the SUs at the end of horizon. As expected, the SUs using SCNJ2$^*$ algorithm suffer highest number of collisions due to sequential hopping in top $N$ channels out of which $J$ channels are jammed by jammers. The number of collisions in myopic algorithm are slightly more than the SCNJ2 algorithm though the SUs in latter sequentially hops in the top $N+J$ channels compared to the SCNJ2 algorithm where the SUs sequentially hops in top $N+m$ channels, where $m\leq J$. This is because, $N+J$ estimation in the myopic algorithm may not be same at all SUs leading to frequent collisions among the SUs. The proposed algorithms guarantee accurate estimation of $N$ and $J$ with a high probability and hence, offers superior performance in terms of throughput as well as number of collisions (hence, longer battery life at SUs). 

%The SUs and jammers are realized using MATLAB and USRP from Ettus Research. 


%\begin{figure*}[!h]
%\centering
%$
%\begin{array}{ccc}
%{\includegraphics[scale=0.275]{N4J2K8_U.pdf}}  &
%{\includegraphics[scale=0.275]{N5J2K8_U.pdf}}  &
%
%{\includegraphics[scale=0.275]{coll.pdf}}
%\end{array}
%$
%\caption {Plot of average regret comparison of SCNJ1 with (a) random strategy (b) $\{N =3,4,5\}$ (c) $\{K=8, 9, 10, ..., 15\}$.}
%	\label{USRP_th}
%\end{figure*}




%\begin{figure*}[htb!]
%\centering
%$
%\begin{array}{ccc}
%{\includegraphics[scale=0.15]{Pics/Model2/ComparisonWithRandom.pdf}}  &
%{\includegraphics[scale=0.15]{Pics/Model2/RegretForDiff_N.pdf}} &
%{\includegraphics[scale=0.15]{Pics/Model2/RegretForDiff_K.pdf}}
%\end{array}
%$
%\caption {Plot of average regret comparison of SCNJ2 with (a) random strategy (b) $\{N =3,4,5\}$ (c) $\{K=8, 9, 10, ..., 15\}$.}
%	\label{fig4}
%
%\end{figure*}
%
%\begin{figure*}[htb!]
%\centering
%$
%\begin{array}{ccc}
%{\includegraphics[scale=0.15]{Pics/Model1/ComparisonWithRandom.pdf}}  &
%{\includegraphics[scale=0.15]{Pics/Model1/RegretForDiff_N.pdf}} &
%{\includegraphics[scale=0.15]{Pics/Model1/RegretForDiff_K.pdf}}
%\end{array}
%$
%\caption {Plot of average regret comparison of SCNJ3 with (a) random strategy (b) $\{N =3,4,5\}$ (c) $\{K=8, 9, 10, ..., 15\}$.}
%	\label{fig5}
%
%\end{figure*}
%

